Liveness Detection in Computer Vision: Transformer-based Self-Supervised Learning for Face Anti-Spoofing

Face recognition systems are increasingly used in biometric security for convenience and effectiveness. However, they remain vulnerable to spoofing attacks, where attackers use photos, videos, or masks to impersonate legitimate users. This research addresses these vulnerabilities by exploring the Vision Transformer (ViT) architecture, fine-tuned with the DINO framework. The DINO framework facilitates self-supervised learning, enabling the model to learn distinguishing features from unlabeled data. We compared the performance of the proposed fine-tuned ViT model using the DINO framework against a traditional CNN model, EfficientNet b2, on the face anti-spoofing task. Numerous tests on standard datasets show that the ViT model performs better than the CNN model in terms of accuracy and resistance to different spoofing methods. Additionally, we collected our own dataset from a biometric application to validate our findings further. This study highlights the superior performance of transformer-based architecture in identifying complex spoofing cues, leading to significant advancements in biometric security.

==> ___colors_and_instructions.tex <==
ADDED (text is part of text)
\textcolor{BrickRed}{} 

CORRECT
\colorbox{Dandelion}{orange background}

IDEA (just idea)
\colorbox{Lavender}{IDEa is great}

If you add the new text after my pravkas, please use a different color—not black and not brick red.

In case you fix the CORRECT, please, change color from Dandelion to Green

All proofreads done by me. Proofread includes paraphrasing and improving the text where needed,fixing language, grammar, checking the use of AI and minimizing it

==> sections/introduction.tex <==
\subsection{Authors and Affiliations}
\textbf{The class file is designed for, but not limited to, six authors.} A 
minimum of one author is required for all conference articles. Author names 
should be listed starting from left to right and then moving down to the 
next line. This is the author sequence that will be used in future citations 
and by indexing services. Names should not be listed in columns nor group by 
affiliation. Please keep your affiliations as succinct as possible (for 
example, do not differentiate among departments of the same organization).


==> sections/references.tex <==
\bibitem{b1} G. Eason, B. Noble, and I. N. Sneddon, ``On certain integrals of Lipschitz-Hankel type involving products of Bessel functions,'' Phil. Trans. Roy. Soc. London, vol. A247, pp. 529--551, April 1955.
